A SPHEREx Pipeline and Spectral Library for Ultracool Dwarfs

We present a Python spectrophotometry extraction tool tailored for fast-moving point sources detected in the SPHEREx mission, and use it to construct a set of 0.75-5.0 $\mu$m low-resolution ($\lambda/\Delta\lambda \sim 50$) spectrophotometry data products based on the SPHEREx Quick Release 2 (QR2) for a set of 6003 L0-Y1 ultracool dwarfs: 2050 known ultracool dwarfs, 3008 known photometric ultracool dwarf candidates, and 947 newly identified ultracool dwarfs. This work more than doubles the number of ultracool dwarfs with spectroscopy, from 3449 to 7402. We provide SPHEREx templates for each spectral subtype and a set of tools to assign automated spectral types. The QR2 data release generates spectrophotometry with an average signal-to-noise per spectral channel above $\sim$10 for most objects with WISE W2 magnitudes of 14.0 mag and brighter. The compiled data set is made available publicly at https://mocadb.ca, where new spectral compilations from future data releases will also be made available as they are published. These new data provide a significant increase in the number of substellar objects for which the 2.4-5.0 $\mu$m window is now accessible, making it possible to probe important molecular chemistry of key CNOS-bearing species for the coolest brown dwarfs. We flag 2668 ultracool dwarfs as candidate young brown dwarfs, 250 as candidate subdwarfs, and 865 as possibly otherwise peculiar for future investigation. The SPIFF library presented here opens the doors to efficient confirmation of candidate substellar objects and follow-up studies of population-level atmospheric properties of cold brown dwarfs.

==> tables/data_spherex_spectra_spiff_columns.tex <==
\begin{tabular}{rclc}
\hline
\textbf{Column} & \textbf{Datatype} & \textbf{Description}\\
\hline
id & bigint(20) unsigned & Auto-increment primary key for this SPIFF result row. \\
md5\_uid & varchar(32) & Deterministic MD5 UID built from pipeline version, object identity, observation IDs, detector/bandpass, and projected reference coordinates. \\
moca\_oid & int(10) unsigned & MOCA object identifier (foreign key to moca\_objects.moca\_oid). \\
moca\_specid & int(10) unsigned & MOCA spectrum identifier linked to this SPIFF row when available (foreign key to moca\_spectra.moca\_specid). \\
target\_name & varchar(255) & Human-readable target name passed to LV2 for this run. \\
reference\_ra\_deg & double & Reference right ascension in degrees used for PM projection / matching. \\
reference\_dec\_deg & double & Reference declination in degrees used for PM projection / matching. \\
reference\_crd\_epoch\_yr & double & Epoch (year) of the reference sky coordinates. \\
reference\_pmra\_masyr & double & Reference proper motion in RA*cos(Dec), in mas/yr. \\
reference\_pmdec\_masyr & double & Reference proper motion in Dec, in mas/yr. \\
input\_ra\_deg & double & RA in degrees actually sent to the image analyzer for this row. \\
input\_dec\_deg & double & Dec in degrees actually sent to the image analyzer for this row. \\
fit\_radius\_px & float & Radial size of the fitting aperture/window in detector pixels. \\
box\_size\_bcg\_subtract & int(11) & Background-subtraction box size (pixels) used around the target. \\
fits\_path & varchar(1024) & Local filesystem path of the FITS file analyzed. \\
access\_url & varchar(1024) & Remote archive URL used to download/access the FITS file. \\
fits\_analysis\_status & varchar(32) & Compact per-image processing status from the LV2 wrapper (success/failure category). \\
analyzer\_stdout & varchar(1024) & Path to captured analyzer stdout log for this row (or inline snippet in failure cases). \\
obs\_collection & varchar(64) & ObsCore collection label for the exposure (e.g. spherex\_qr2). \\
obsid & varchar(64) & SPHEREx observation identifier from FITS/ObsCore. \\
bandpass & varchar(60) & Bandpass/detector channel label (e.g. D1..D6). \\
expid & varchar(64) & Exposure identifier for the image frame. \\
mjd\_avg & double & Average MJD timestamp of the exposure. \\
detector\_id & int(11) & Numeric detector/channel ID from FITS metadata. \\
psf\_index & int(11) & Index of the PSF kernel selected from the PSF cube. \\
omega\_sr & double & Median detector-pixel solid angle in steradians. \\
px\_scale\_arcsec & double & Detector pixel scale in arcsec/pixel. \\
near\_cutout\_edge & tinyint(1) & Boolean flag indicating source is near the edge of the extracted cutout. \\
near\_detector\_edge & tinyint(1) & Boolean flag indicating source is near detector image boundaries. \\
near\_bcg\_star & tinyint(1) & Boolean flag indicating proximity to bright contaminating source/background structure. \\
n\_pix\_flagged\_in\_fit & int(11) & Number of pixels excluded by masking/flags inside the fit region. \\
n\_pix\_used\_in\_fit & int(11) & Number of valid pixels used by the fit in the fit region. \\
n\_pix\_total\_in\_fit & int(11) & Total pixels in the fit region before masking. \\
ap\_radius\_px & float & Aperture-photometry radius in pixels. \\
ap\_radius\_forced & tinyint(1) & Boolean: aperture radius was forced/clipped instead of nominal automatic value. \\
ap\_flux\_MJysr & float & Aperture flux density in MJy/sr (background-subtracted). \\
ap\_flux\_MJysr\_err & float & Uncertainty on aperture flux density in MJy/sr. \\
ap\_snr & float & Signal-to-noise ratio from aperture photometry. \\
ap\_centroid\_err\_px & float & Estimated centroid uncertainty for aperture-based position, in pixels. \\
ap\_flux\_uJy & float & Aperture integrated flux in microJy. \\
ap\_flux\_uJy\_err & float & Uncertainty on aperture integrated flux in microJy. \\
ap\_xcen\_cutout & double & Aperture centroid X coordinate in cutout pixel frame. \\
ap\_ycen\_cutout & double & Aperture centroid Y coordinate in cutout pixel frame. \\
ap\_xcen\_fullim & double & Aperture centroid X coordinate in full-image pixel frame. \\
ap\_ycen\_fullim & double & Aperture centroid Y coordinate in full-image pixel frame. \\
com\_xcen\_cutout & double & Center-of-mass X coordinate in cutout pixel frame. \\
com\_ycen\_cutout & double & Center-of-mass Y coordinate in cutout pixel frame. \\
com\_xcen\_fullim & double & Center-of-mass X coordinate in full-image pixel frame. \\
com\_ycen\_fullim & double & Center-of-mass Y coordinate in full-image pixel frame. \\
com\_ra\_deg & double & Center-of-mass sky RA in degrees. \\
com\_dec\_deg & double & Center-of-mass sky Dec in degrees. \\
com\_sep\_as & double & Angular separation between COM position and input target position, in arcsec. \\
com\_wv\_um & double & Interpolated central wavelength at COM position from WCS-WAVE, in microns. \\
com\_wv\_width\_um & double & Interpolated channel width (effective bandpass width) at COM position, in microns. \\
psf\_scipy\_method\_used & varchar(64) & Optimizer method string reported by the scipy psf fit stage. \\
psf\_scipy\_status & varchar(64) & Optimizer status/message reported by the scipy psf fit stage. \\
psf\_scipy\_flux\_MJysr & float & SciPy PSF fit flux density amplitude in MJy/sr. \\
psf\_scipy\_flux\_MJysr\_err & float & Uncertainty on scipy psf fit flux density amplitude in MJy/sr. \\
psf\_scipy\_snr & float & Signal-to-noise ratio from the scipy psf fit solution. \\
psf\_scipy\_flux\_uJy & float & SciPy PSF fit integrated flux in microJy. \\
psf\_scipy\_flux\_uJy\_err & float & Uncertainty on scipy psf fit integrated flux in microJy. \\
psf\_scipy\_dx & float & SciPy PSF fit best-fit X offset relative to target center, in cutout pixels. \\
psf\_scipy\_dy & float & SciPy PSF fit best-fit Y offset relative to target center, in cutout pixels. \\
psf\_scipy\_xcen\_cutout & double & SciPy PSF fit centroid X coordinate in cutout pixel frame. \\
psf\_scipy\_ycen\_cutout & double & SciPy PSF fit centroid Y coordinate in cutout pixel frame. \\
psf\_scipy\_xcen\_fullim & double & SciPy PSF fit centroid X coordinate in full-image pixel frame. \\
psf\_scipy\_ycen\_fullim & double & SciPy PSF fit centroid Y coordinate in full-image pixel frame. \\
psf\_scipy\_ra\_deg & double & SciPy PSF fit sky RA in degrees. \\
psf\_scipy\_ra\_err\_mas & double & Uncertainty on scipy psf fit RA, in mas. \\
psf\_scipy\_dec\_deg & double & SciPy PSF fit sky Dec in degrees. \\
psf\_scipy\_dec\_err\_mas & double & Uncertainty on scipy psf fit Dec, in mas. \\
psf\_scipy\_ra\_dec\_cov\_mas2 & double & RA/Dec covariance from scipy psf fit uncertainty propagation, in mas\textasciicircum{}2. \\
psf\_scipy\_sep\_as & double & Angular separation between scipy psf fit position and input target, in arcsec. \\
psf\_scipy\_wv\_um & double & Central wavelength at scipy psf fit centroid from WCS-WAVE, in microns. \\
psf\_scipy\_wv\_um\_err & double & Uncertainty on central wavelength for scipy psf fit centroid, in microns. \\
psf\_scipy\_wv\_width\_um & double & Bandpass width at scipy psf fit centroid from WCS-WAVE, in microns. \\
psf\_scipy\_wv\_width\_um\_err & double & Uncertainty on bandpass width for scipy psf fit centroid, in microns. \\
psf\_scipy\_chi2 & double & Chi-square goodness-of-fit value for the scipy psf fit solution. \\
psf\_scipy\_dof & int(11) & Degrees of freedom used for chi-square in the scipy psf fit solution. \\
psf\_un\_flux\_MJysr & float & UltraNest PSF fit flux density amplitude in MJy/sr. \\
psf\_un\_flux\_MJysr\_err & float & Uncertainty on ultranest psf fit flux density amplitude in MJy/sr. \\
psf\_un\_snr & float & Signal-to-noise ratio from the ultranest psf fit solution. \\
psf\_un\_flux\_uJy & float & UltraNest PSF fit integrated flux in microJy. \\
psf\_un\_flux\_uJy\_err & float & Uncertainty on ultranest psf fit integrated flux in microJy. \\
psf\_un\_dx & float & UltraNest PSF fit best-fit X offset relative to target center, in cutout pixels. \\
psf\_un\_dy & float & UltraNest PSF fit best-fit Y offset relative to target center, in cutout pixels. \\
psf\_un\_xcen\_cutout & double & UltraNest PSF fit centroid X coordinate in cutout pixel frame. \\
psf\_un\_ycen\_cutout & double & UltraNest PSF fit centroid Y coordinate in cutout pixel frame. \\
psf\_un\_xcen\_fullim & double & UltraNest PSF fit centroid X coordinate in full-image pixel frame. \\
psf\_un\_ycen\_fullim & double & UltraNest PSF fit centroid Y coordinate in full-image pixel frame. \\
psf\_un\_xcen\_err & double & Uncertainty on ultranest psf fit centroid X in pixels. \\
psf\_un\_ycen\_err & double & Uncertainty on ultranest psf fit centroid Y in pixels. \\
psf\_un\_ra\_deg & double & UltraNest PSF fit sky RA in degrees. \\
psf\_un\_ra\_err\_mas & double & Uncertainty on ultranest psf fit RA, in mas. \\
psf\_un\_dec\_deg & double & UltraNest PSF fit sky Dec in degrees. \\
psf\_un\_dec\_err\_mas & double & Uncertainty on ultranest psf fit Dec, in mas. \\
psf\_un\_sep\_as & double & Angular separation between ultranest psf fit position and input target, in arcsec. \\
psf\_un\_ra\_dec\_cov\_mas2 & double & RA/Dec covariance from ultranest psf fit uncertainty propagation, in mas\textasciicircum{}2. \\
psf\_un\_wv\_um & double & Central wavelength at ultranest psf fit centroid from WCS-WAVE, in microns. \\
psf\_un\_wv\_um\_err & double & Uncertainty on central wavelength for ultranest psf fit centroid, in microns. \\
psf\_un\_wv\_width\_um & double & Bandpass width at ultranest psf fit centroid from WCS-WAVE, in microns. \\
psf\_un\_wv\_width\_um\_err & double & Uncertainty on bandpass width for ultranest psf fit centroid, in microns. \\
psf\_un\_chi2 & double & Chi-square goodness-of-fit value for the ultranest psf fit solution. \\
psf\_un\_dof & int(11) & Degrees of freedom used for chi-square in the ultranest psf fit solution. \\
ignored & tinyint(1) & Boolean soft-delete/ignore flag for downstream usage. \\
calculation\_method & varchar(60) & Processing method label; for this pipeline typically SPIFF. \\
origin & varchar(255) & Origin tag of producer code (e.g. lv2\_wrapper). \\
pipeline\_version & varchar(64) & Pipeline version string associated with this row. \\
modified\_timestamp & timestamp & Row last-modified timestamp (auto-updated). \\
comments & text & Free-text comment field (often populated from fits\_analysis\_comment/failure reason). \\
created\_timestamp & timestamp & Row creation timestamp. \\
no\_masking & tinyint(1) & If 1, PSF-fit flag-based masking was disabled (--no-masking). \\
\hline
\end{tabular}


==> tables/data_spherex_spectra_spiff_fulltable.tex <==
\startlongtable
\begin{deluxetable*}{lll}
\tablecaption{Columns in \texttt{data\_spherex\_spectra\_spiff}}
\label{tab:spiff}
\tablehead{
\colhead{Column} & \colhead{Datatype} & \colhead{Description}
}
\startdata
id & bigint(20) unsigned & Primary identifier for this row. \\
md5\_uid & varchar(32) & Deterministic MD5 UID built from pipeline version, object identity, observation IDs, detector/bandpass, and projected reference coordinates. \\
moca\_oid & int(10) unsigned & MOCA object identifier (foreign key to moca\_objects.moca\_oid). \\
moca\_specid & int(10) unsigned & MOCA spectrum identifier linked to this SPIFF row when available (foreign key to moca\_spectra.moca\_specid). \\
target\_name & varchar(255) & Human-readable target name passed to LV2 for this run. \\
reference\_ra\_deg & double & Reference right ascension in degrees used for PM projection / matching. \\
reference\_dec\_deg & double & Reference declination in degrees used for PM projection / matching. \\
reference\_crd\_epoch\_yr & double & Epoch (year) of the reference sky coordinates. \\
reference\_pmra\_masyr & double & Reference proper motion in RA*cos(Dec), in mas/yr. \\
reference\_pmdec\_masyr & double & Reference proper motion in Dec, in mas/yr. \\
input\_ra\_deg & double & RA in degrees actually sent to the image analyzer for this row. \\
input\_dec\_deg & double & Dec in degrees actually sent to the image analyzer for this row. \\
fit\_radius\_px & float & Radial size of the fitting aperture/window in detector pixels. \\
box\_size\_bcg\_subtract & int(11) & Background-subtraction box size (pixels) used around the target. \\
fits\_path & varchar(1024) & Local filesystem path of the FITS file analyzed. \\
access\_url & varchar(1024) & Remote archive URL used to download/access the FITS file. \\
fits\_analysis\_status & varchar(32) & Compact per-image processing status from the LV2 wrapper (success/failure category). \\
analyzer\_stdout & varchar(1024) & Path to captured analyzer stdout log for this row (or inline snippet in failure cases). \\
obs\_collection & varchar(64) & ObsCore collection label for the exposure (e.g. spherex\_qr2). \\
obsid & varchar(64) & SPHEREx observation identifier from FITS/ObsCore. \\
bandpass & varchar(60) & Bandpass/detector channel label (e.g. D1..D6). \\
expid & varchar(64) & Exposure identifier for the image frame. \\
mjd\_avg & double & Average MJD timestamp of the exposure. \\
detector\_id & int(11) & Numeric detector/channel ID from FITS metadata. \\
psf\_index & int(11) & Index of the PSF kernel selected from the PSF cube. \\
omega\_sr & double & Median detector-pixel solid angle in steradians. \\
px\_scale\_arcsec & double & Detector pixel scale in arcsec/pixel. \\
near\_cutout\_edge & tinyint(1) & Boolean flag indicating source is near the edge of the extracted cutout. \\
near\_detector\_edge & tinyint(1) & Boolean flag indicating source is near detector image boundaries. \\
near\_bcg\_star & tinyint(1) & Boolean flag indicating proximity to bright contaminating source/background structure. \\
n\_pix\_flagged\_in\_fit & int(11) & Number of pixels excluded by masking/flags inside the fit region. \\
n\_pix\_used\_in\_fit & int(11) & Number of valid pixels used by the fit in the fit region. \\
n\_pix\_total\_in\_fit & int(11) & Total pixels in the fit region before masking. \\
ap\_radius\_px & float & Aperture-photometry radius in pixels. \\
ap\_radius\_forced & tinyint(1) & Boolean: aperture radius was forced/clipped instead of nominal automatic value. \\
ap\_flux\_MJysr & float & Aperture flux density in MJy/sr (background-subtracted). \\
ap\_flux\_MJysr\_err & float & Uncertainty on aperture flux density in MJy/sr. \\
ap\_snr & float & Signal-to-noise ratio from aperture photometry. \\
ap\_centroid\_err\_px & float & Estimated centroid uncertainty for aperture-based position, in pixels. \\
ap\_flux\_uJy & float & Aperture integrated flux in microJy. \\
ap\_flux\_uJy\_err & float & Uncertainty on aperture integrated flux in microJy. \\
ap\_xcen\_cutout & double & Aperture centroid X coordinate in cutout pixel frame. \\
ap\_ycen\_cutout & double & Aperture centroid Y coordinate in cutout pixel frame. \\
ap\_xcen\_fullim & double & Aperture centroid X coordinate in full-image pixel frame. \\
ap\_ycen\_fullim & double & Aperture centroid Y coordinate in full-image pixel frame. \\
com\_xcen\_cutout & double & Center-of-mass X coordinate in cutout pixel frame. \\
com\_ycen\_cutout & double & Center-of-mass Y coordinate in cutout pixel frame. \\
com\_xcen\_fullim & double & Center-of-mass X coordinate in full-image pixel frame. \\
com\_ycen\_fullim & double & Center-of-mass Y coordinate in full-image pixel frame. \\
com\_ra\_deg & double & Center-of-mass sky RA in degrees. \\
com\_dec\_deg & double & Center-of-mass sky Dec in degrees. \\
com\_sep\_as & double & Angular separation between COM position and input target position, in arcsec. \\
com\_wv\_um & double & Interpolated central wavelength at COM position from WCS-WAVE, in microns. \\
com\_wv\_width\_um & double & Interpolated channel width (effective bandpass width) at COM position, in microns. \\
psf\_scipy\_method\_used & varchar(64) & Optimizer method string reported by the scipy psf fit stage. \\
psf\_scipy\_status & varchar(64) & Optimizer status/message reported by the scipy psf fit stage. \\
psf\_scipy\_flux\_MJysr & float & SciPy PSF fit flux density amplitude in MJy/sr. \\
psf\_scipy\_flux\_MJysr\_err & float & Uncertainty on scipy psf fit flux density amplitude in MJy/sr. \\
psf\_scipy\_snr & float & Signal-to-noise ratio from the scipy psf fit solution. \\
psf\_scipy\_flux\_uJy & float & SciPy PSF fit integrated flux in microJy. \\
psf\_scipy\_flux\_uJy\_err & float & Uncertainty on scipy psf fit integrated flux in microJy. \\
psf\_scipy\_dx & float & SciPy PSF fit best-fit X offset relative to target center, in cutout pixels. \\
psf\_scipy\_dy & float & SciPy PSF fit best-fit Y offset relative to target center, in cutout pixels. \\
psf\_scipy\_xcen\_cutout & double & SciPy PSF fit centroid X coordinate in cutout pixel frame. \\
psf\_scipy\_ycen\_cutout & double & SciPy PSF fit centroid Y coordinate in cutout pixel frame. \\
psf\_scipy\_xcen\_fullim & double & SciPy PSF fit centroid X coordinate in full-image pixel frame. \\
psf\_scipy\_ycen\_fullim & double & SciPy PSF fit centroid Y coordinate in full-image pixel frame. \\
psf\_scipy\_ra\_deg & double & SciPy PSF fit sky RA in degrees. \\
psf\_scipy\_ra\_err\_mas & double & Uncertainty on scipy psf fit RA, in mas. \\
psf\_scipy\_dec\_deg & double & SciPy PSF fit sky Dec in degrees. \\
psf\_scipy\_dec\_err\_mas & double & Uncertainty on scipy psf fit Dec, in mas. \\
psf\_scipy\_ra\_dec\_cov\_mas2 & double & RA/Dec covariance from scipy psf fit uncertainty propagation, in mas\textasciicircum{}2. \\
psf\_scipy\_sep\_as & double & Angular separation between scipy psf fit position and input target, in arcsec. \\
psf\_scipy\_wv\_um & double & Central wavelength at scipy psf fit centroid from WCS-WAVE, in microns. \\
psf\_scipy\_wv\_um\_err & double & Uncertainty on central wavelength for scipy psf fit centroid, in microns. \\
psf\_scipy\_wv\_width\_um & double & Bandpass width at scipy psf fit centroid from WCS-WAVE, in microns. \\
psf\_scipy\_wv\_width\_um\_err & double & Uncertainty on bandpass width for scipy psf fit centroid, in microns. \\
psf\_scipy\_chi2 & double & Chi-square goodness-of-fit value for the scipy psf fit solution. \\
psf\_scipy\_dof & int(11) & Degrees of freedom used for chi-square in the scipy psf fit solution. \\
psf\_un\_flux\_MJysr & float & UltraNest PSF fit flux density amplitude in MJy/sr. \\
psf\_un\_flux\_MJysr\_err & float & Uncertainty on ultranest psf fit flux density amplitude in MJy/sr. \\
psf\_un\_snr & float & Signal-to-noise ratio from the ultranest psf fit solution. \\
psf\_un\_flux\_uJy & float & UltraNest PSF fit integrated flux in microJy. \\
psf\_un\_flux\_uJy\_err & float & Uncertainty on ultranest psf fit integrated flux in microJy. \\
psf\_un\_dx & float & UltraNest PSF fit best-fit X offset relative to target center, in cutout pixels. \\
psf\_un\_dy & float & UltraNest PSF fit best-fit Y offset relative to target center, in cutout pixels. \\
psf\_un\_xcen\_cutout & double & UltraNest PSF fit centroid X coordinate in cutout pixel frame. \\
psf\_un\_ycen\_cutout & double & UltraNest PSF fit centroid Y coordinate in cutout pixel frame. \\
psf\_un\_xcen\_fullim & double & UltraNest PSF fit centroid X coordinate in full-image pixel frame. \\
psf\_un\_ycen\_fullim & double & UltraNest PSF fit centroid Y coordinate in full-image pixel frame. \\
psf\_un\_xcen\_err & double & Uncertainty on ultranest psf fit centroid X in pixels. \\
psf\_un\_ycen\_err & double & Uncertainty on ultranest psf fit centroid Y in pixels. \\
psf\_un\_ra\_deg & double & UltraNest PSF fit sky RA in degrees. \\
psf\_un\_ra\_err\_mas & double & Uncertainty on ultranest psf fit RA, in mas. \\
psf\_un\_dec\_deg & double & UltraNest PSF fit sky Dec in degrees. \\
psf\_un\_dec\_err\_mas & double & Uncertainty on ultranest psf fit Dec, in mas. \\
psf\_un\_sep\_as & double & Angular separation between ultranest psf fit position and input target, in arcsec. \\
psf\_un\_ra\_dec\_cov\_mas2 & double & RA/Dec covariance from ultranest psf fit uncertainty propagation, in mas\textasciicircum{}2. \\
psf\_un\_wv\_um & double & Central wavelength at ultranest psf fit centroid from WCS-WAVE, in microns. \\
psf\_un\_wv\_um\_err & double & Uncertainty on central wavelength for ultranest psf fit centroid, in microns. \\
psf\_un\_wv\_width\_um & double & Bandpass width at ultranest psf fit centroid from WCS-WAVE, in microns. \\
psf\_un\_wv\_width\_um\_err & double & Uncertainty on bandpass width for ultranest psf fit centroid, in microns. \\
psf\_un\_chi2 & double & Chi-square goodness-of-fit value for the ultranest psf fit solution. \\
psf\_un\_dof & int(11) & Degrees of freedom used for chi-square in the ultranest psf fit solution. \\
ignored & tinyint(1) & Boolean soft-delete/ignore flag for downstream usage. \\
calculation\_method & varchar(60) & Processing method label; for this pipeline typically SPIFF. \\
origin & varchar(255) & Origin tag of producer code (e.g. lv2\_wrapper). \\
pipeline\_version & varchar(64) & Pipeline version string associated with this row. \\
modified\_timestamp & timestamp & Row last-modified timestamp (auto-updated). \\
comments & text & Free-text comment field (often populated from fits\_analysis\_comment/failure reason). \\
created\_timestamp & timestamp & Row creation timestamp. \\
no\_masking & tinyint(1) & If 1, PSF-fit flag-based masking was disabled (--no-masking). \\
\enddata
\end{deluxetable*}


==> tables/pcat_spherex_bins_bandpasses.tex <==
\startlongtable
\begin{deluxetable}{cll}
\tablecaption{SPHEREx Channel Centers and Widths\label{tab:bandpass}}
\tablehead{
\colhead{Index} & \colhead{$\lambda_{\mathrm{center}}$ ($\mu$m)} & \colhead{$\lambda_{\mathrm{width}}$ ($\mu$m)}
}
\startdata
1 & 0.744 & 0.022 \\
2 & 0.766 & 0.022 \\
3 & 0.788 & 0.022 \\
4 & 0.810 & 0.022 \\
5 & 0.832 & 0.022 \\
6 & 0.853 & 0.022 \\
7 & 0.875 & 0.022 \\
8 & 0.897 & 0.022 \\
9 & 0.919 & 0.022 \\
10 & 0.941 & 0.022 \\
11 & 0.963 & 0.022 \\
12 & 0.985 & 0.022 \\
13 & 1.007 & 0.022 \\
14 & 1.028 & 0.022 \\
15 & 1.050 & 0.022 \\
16 & 1.072 & 0.022 \\
17 & 1.094 & 0.022 \\
18 & 1.099 & 0.032 \\
19 & 1.131 & 0.032 \\
20 & 1.164 & 0.032 \\
21 & 1.196 & 0.032 \\
22 & 1.229 & 0.032 \\
23 & 1.261 & 0.032 \\
24 & 1.294 & 0.032 \\
25 & 1.326 & 0.032 \\
26 & 1.359 & 0.032 \\
27 & 1.391 & 0.032 \\
28 & 1.424 & 0.032 \\
29 & 1.456 & 0.032 \\
30 & 1.489 & 0.032 \\
31 & 1.521 & 0.032 \\
32 & 1.554 & 0.032 \\
33 & 1.586 & 0.032 \\
34 & 1.619 & 0.032 \\
35 & 1.636 & 0.046 \\
36 & 1.682 & 0.046 \\
37 & 1.728 & 0.046 \\
38 & 1.775 & 0.046 \\
39 & 1.821 & 0.046 \\
40 & 1.867 & 0.046 \\
41 & 1.913 & 0.046 \\
42 & 1.959 & 0.046 \\
43 & 2.005 & 0.046 \\
44 & 2.052 & 0.046 \\
45 & 2.098 & 0.046 \\
46 & 2.144 & 0.046 \\
47 & 2.190 & 0.046 \\
48 & 2.236 & 0.046 \\
49 & 2.282 & 0.046 \\
50 & 2.329 & 0.046 \\
51 & 2.375 & 0.046 \\
52 & 2.423 & 0.082 \\
53 & 2.505 & 0.082 \\
54 & 2.588 & 0.082 \\
55 & 2.670 & 0.082 \\
56 & 2.752 & 0.082 \\
57 & 2.834 & 0.082 \\
58 & 2.917 & 0.082 \\
59 & 2.999 & 0.082 \\
60 & 3.081 & 0.082 \\
61 & 3.164 & 0.082 \\
62 & 3.246 & 0.082 \\
63 & 3.328 & 0.082 \\
64 & 3.411 & 0.082 \\
65 & 3.493 & 0.082 \\
66 & 3.575 & 0.082 \\
67 & 3.657 & 0.082 \\
68 & 3.740 & 0.082 \\
69 & 3.809 & 0.036 \\
70 & 3.845 & 0.036 \\
71 & 3.881 & 0.036 \\
72 & 3.917 & 0.036 \\
73 & 3.953 & 0.036 \\
74 & 3.989 & 0.036 \\
75 & 4.025 & 0.036 \\
76 & 4.061 & 0.036 \\
77 & 4.097 & 0.036 \\
78 & 4.132 & 0.036 \\
79 & 4.168 & 0.036 \\
80 & 4.204 & 0.036 \\
81 & 4.240 & 0.036 \\
82 & 4.276 & 0.036 \\
83 & 4.312 & 0.036 \\
84 & 4.348 & 0.036 \\
85 & 4.384 & 0.036 \\
86 & 4.412 & 0.035 \\
87 & 4.447 & 0.035 \\
88 & 4.481 & 0.035 \\
89 & 4.516 & 0.035 \\
90 & 4.551 & 0.035 \\
91 & 4.586 & 0.035 \\
92 & 4.620 & 0.035 \\
93 & 4.655 & 0.035 \\
94 & 4.690 & 0.035 \\
95 & 4.724 & 0.035 \\
96 & 4.759 & 0.035 \\
97 & 4.794 & 0.035 \\
98 & 4.828 & 0.035 \\
99 & 4.863 & 0.035 \\
100 & 4.898 & 0.035 \\
101 & 4.933 & 0.035 \\
102 & 4.967 & 0.035 \\
\enddata
\end{deluxetable}


==> tables/pcat_spherex_bins_bandpasses_fulltable.tex <==
\startlongtable
\begin{deluxetable}{cll}
\tablewidth{\textwidth}
\tablecaption{Preliminary SPHEREx channel characteristics (Full Table)\label{tab:bandpass}}
\tablehead{
\colhead{Index} & \colhead{$\lambda_{\mathrm{center}}$ ($\mu$m)} & \colhead{$\lambda_{\mathrm{width}}$ ($\mu$m)}
}
\startdata
1 & 0.744 & 0.022 \\
2 & 0.766 & 0.022 \\
3 & 0.788 & 0.022 \\
4 & 0.810 & 0.022 \\
5 & 0.832 & 0.022 \\
6 & 0.853 & 0.022 \\
7 & 0.875 & 0.022 \\
8 & 0.897 & 0.022 \\
9 & 0.919 & 0.022 \\
10 & 0.941 & 0.022 \\
11 & 0.963 & 0.022 \\
12 & 0.985 & 0.022 \\
13 & 1.007 & 0.022 \\
14 & 1.028 & 0.022 \\
15 & 1.050 & 0.022 \\
16 & 1.072 & 0.022 \\
17 & 1.094 & 0.022 \\
18 & 1.099 & 0.032 \\
19 & 1.131 & 0.032 \\
20 & 1.164 & 0.032 \\
21 & 1.196 & 0.032 \\
22 & 1.229 & 0.032 \\
23 & 1.261 & 0.032 \\
24 & 1.294 & 0.032 \\
25 & 1.326 & 0.032 \\
26 & 1.359 & 0.032 \\
27 & 1.391 & 0.032 \\
28 & 1.424 & 0.032 \\
29 & 1.456 & 0.032 \\
30 & 1.489 & 0.032 \\
31 & 1.521 & 0.032 \\
32 & 1.554 & 0.032 \\
33 & 1.586 & 0.032 \\
34 & 1.619 & 0.032 \\
35 & 1.636 & 0.046 \\
36 & 1.682 & 0.046 \\
37 & 1.728 & 0.046 \\
38 & 1.775 & 0.046 \\
39 & 1.821 & 0.046 \\
40 & 1.867 & 0.046 \\
41 & 1.913 & 0.046 \\
42 & 1.959 & 0.046 \\
43 & 2.005 & 0.046 \\
44 & 2.052 & 0.046 \\
45 & 2.098 & 0.046 \\
46 & 2.144 & 0.046 \\
47 & 2.190 & 0.046 \\
48 & 2.236 & 0.046 \\
49 & 2.282 & 0.046 \\
50 & 2.329 & 0.046 \\
51 & 2.375 & 0.046 \\
52 & 2.423 & 0.082 \\
53 & 2.505 & 0.082 \\
54 & 2.588 & 0.082 \\
55 & 2.670 & 0.082 \\
56 & 2.752 & 0.082 \\
57 & 2.834 & 0.082 \\
58 & 2.917 & 0.082 \\
59 & 2.999 & 0.082 \\
60 & 3.081 & 0.082 \\
61 & 3.164 & 0.082 \\
62 & 3.246 & 0.082 \\
63 & 3.328 & 0.082 \\
64 & 3.411 & 0.082 \\
65 & 3.493 & 0.082 \\
66 & 3.575 & 0.082 \\
67 & 3.657 & 0.082 \\
68 & 3.740 & 0.082 \\
69 & 3.809 & 0.036 \\
70 & 3.845 & 0.036 \\
71 & 3.881 & 0.036 \\
72 & 3.917 & 0.036 \\
73 & 3.953 & 0.036 \\
74 & 3.989 & 0.036 \\
75 & 4.025 & 0.036 \\
76 & 4.061 & 0.036 \\
77 & 4.097 & 0.036 \\
78 & 4.132 & 0.036 \\
79 & 4.168 & 0.036 \\
80 & 4.204 & 0.036 \\
81 & 4.240 & 0.036 \\
82 & 4.276 & 0.036 \\
83 & 4.312 & 0.036 \\
84 & 4.348 & 0.036 \\
85 & 4.384 & 0.036 \\
86 & 4.412 & 0.035 \\
87 & 4.447 & 0.035 \\
88 & 4.481 & 0.035 \\
89 & 4.516 & 0.035 \\
90 & 4.551 & 0.035 \\
91 & 4.586 & 0.035 \\
92 & 4.620 & 0.035 \\
93 & 4.655 & 0.035 \\
94 & 4.690 & 0.035 \\
95 & 4.724 & 0.035 \\
96 & 4.759 & 0.035 \\
97 & 4.794 & 0.035 \\
98 & 4.828 & 0.035 \\
99 & 4.863 & 0.035 \\
100 & 4.898 & 0.035 \\
101 & 4.933 & 0.035 \\
102 & 4.967 & 0.035 \\
\enddata
\end{deluxetable}

